Safety verification of asynchronous pushdown systems with shaped stacks

In this paper, we study the program-point reachability problem of concurrent pushdown systems that communicate via unbounded and unordered message buffers. Our goal is to relax the common restriction that messages can only be retrieved by a pushdown process when its stack is empty. We use the notion of partially commutative context-free grammars to describe a new class of asynchronously communicating pushdown systems with a mild shape constraint on the stacks for which the program-point coverability problem remains decidable. Stacks that fit the shape constraint may reach arbitrary heights; further a process may execute any communication action (be it process creation, message send or retrieval) whether or not its stack is empty. This class extends previous computational models studied in the context of asynchronous programs, and enables the safety verification of a large class of message passing programs.

==> figures/pdsmutex.tex <==
%!TEX root = ../main.tex
\begin{multicols}{2}
\begin{erlang}[emph={c1,c2,toResource,toClients,toServer,init,false,true,dist,redist,local,which,globalstate,ready,result}]
%%% Server
server() -> setup_network(), 
            redistribute().

setup_network() ->
  spawn(client),
  case (*) of
    True  -> setup_network();
    False -> 
      spawn(fun() -> resource(c1,c2,init) end),
      toResource ! isReady,
      receive fromResource:
         ready -> ()
      end;
  end, toClients ! task.

redistribute() ->
  receive toServer:
    redist(Task) -> toClients ! Task;
    result(Result) -> print(Result);
  end, redistribute().

%Combinator
combinator(C) ->
  receive C:
    (Res,IRes) -> 
      R = combine_results(Res,IRes),
      toServer ! R
  end,
  combinator(C).

% Resource
resource(C,C',S) ->
  receive toResource:
    which -> toClients ! C, resource(C',C,S);
    lock_req -> toClients ! locked, resource_locked(C,C',S);
  end.

resource_locked(C,C') ->
  receive toResource:
    unlock_req -> resource(C,C',S);
    X          -> resource_locked(C,C',update(S,X))
  end.

%%% Task CLIENT
client() ->
  receive toClients:
    Task -> 
      result = do_task(Task,false),
      case result of
        dist(C) -> ok;
        _       -> to_server ! result
      end;
  end, client().

do_task(Task) ->
  case decompose(Task) of
    local(Task',Int_result) -> 
      Result = do_task(Task'),
      return (combine(Result,Int_result));
    dist(Task', Int_result) -> 
      C = which_combine_resource(),
      Result = do_task(Task'),
      C ! (Result, Int_result),
      return Dist(C);
    redist(Task',Task'') ->  
      result = do_task(Task'),
      to_server ! Redist(Task''),
      return result;
  end.

combine(res,res')    -> combine_results(res,res');
combine(Dist(C),res) -> C ! res.

which_combine_resource() -> 
  resource ! which,
    receive toClients:
      Resource(r) -> return r
    end.

decompose_task(Task) -> 
  lock(toResource),
  resource ! getGlobalstate,
  ?Critical,
  receive toClients: 
    State ->
      (Result,Update) = decompose_task(Task, State)
  end,
  resource ! update(Update),
  unlock(toResource),
  return Result

lock(C)  -> ok;
lock(C) -> 
  C ! lock_req,
  receive toClients:
    locked -> ok
  end.

unlock(C) -> C ! unlock_req.

combine_results(res,res') -> ...

decompose_task(Task,state) -> ...

%%% Program Entry points
main() -> 
  spawn(server),
  spawn(fun() -> combinator(c1) end),
  spawn(fun() -> combinator(c2) end).
  
\end{erlang}
\end{multicols}

==> macros.tex <==
% !TEX root = main.tex
\makeatletter

\def\my@test@bf{bx}

\newcommand{\Soter}{\textsf{Soter}}
\newcommand{\SoterUrl}{\url{http://mjolnir.cs.ox.ac.uk/soter/}}
\newcommand{\BFC}{{BFC}}
\newcommand{\Lang}{%
	\texorpdfstring%
        % {${{\ifx\f@series\my@test@bf\boldsymbol{\lambda}\else\lambda\fi}_{\textup{act}}}$}%
        % {Lambda-act}%
        {${{\ifx\f@series\my@test@bf\boldsymbol{\lambda}\else\lambda\fi}{\textsc{\scriptsize Actor}}}$}%
		{Lambda-Actor}%
        % {${\mathcal{A}_\lambda}$}%
        % {A-lambda}%
}


\mathchardef\breakingcomma\mathcode`\,
{\catcode`,=\active
  \gdef,{\breakingcomma\discretionary{}{}{}}
}
\newcommand{\commabr}[1]{\mathcode`\,=\string"8000 #1}

\newcommand\textbfit[1]{{\bf \emph{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Generic Math operators and abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bigO}[1]{\ensuremath{O(#1)}}

\let\vect\vec
%\renewcommand{\vec}[1]{\mathbf{#1}}
\renewcommand{\vec}[1]{\overrightarrow{#1}}

\newcommand{\sem}[1]{\llbracket#1\rrbracket}

\renewcommand{\P}{\powerset}
\newcommand{\M}{\mathbb{M}}
\newcommand{\bigunion}{\Union}

\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Int}{\mathbb{Z}}
\newcommand{\powerset}{\mathscr{P}}
\newcommand{\finpow}{\powerset_{\!\!f}}
\newcommand{\union}{\cup}
\newcommand{\inters}{\cap}
\newcommand{\Union}{\bigcup}
\newcommand{\Inters}{\bigcap}
\newcommand{\dunion}{\uplus}
\newcommand{\Dunion}{\biguplus}
\providecommand{\implies}{\Rightarrow}
\newcommand{\iif}{\Leftrightarrow}
\newcommand{\iso}{\cong}

\renewcommand\implies{\Rightarrow}

\newcommand{\freevars}{\operatorname{fv}}

% \newcommand{\LeftEqNo}{\let\veqno\@@leqno}

\newcommand{\tuple}[1]{\langle\commabr{#1}\rangle}
\newcommand{\lst}[3][1]{{#2_{#1}}\ldots {#2_{#3}}}    % b_a ... b_c
\newcommand{\lstc}[3][1]{\commabr{{#2_{#1}},\ldots, {#2_{#3}}}} % b_a ,..., b_c
\newcommand{\lsts}[4]{#1_#2#4\ldots#4 #1_{#3}}        % b_a d...d b_c
\newcommand{\vct}[3][]{\ensuremath{\bar #2}} % unused args are intentional so \vect can be redef to be \lst

\newcommand{\is}{\mathrel{\mathop:}=}
%\newcommand{\anglebra}[1]{{\langle #1 \rangle}}
%\newcommand{\preordleq}{\preccurlyeq}
\newcommand\makeset[1]{{ {\{} #1{\}} }}
%\newcommand\arrlab[1]{\stackrel{#1}{\longrightarrow}}
%\newcommand\arr{\rightarrow}
%\newcommand\arrstarlab[1]{\stackrel{#1}{\longrightarrow^{\ast}}}
\newcommand\sendto[2]{{#2 \mathbin{\hbox{!}} #1}}
\newcommand\receivefrom[2]{{#2 \mathbin{\hbox{?}} #1}}
%\newcommand\seq[2]{{{#1} \vdash {#2}}}
%\newcommand{\cpst}[1]{\ensuremath{\left\llbracket#1\right\rrbracket}}
%\newcommand{\cps}[1]{\ensuremath{#1_{\text{cps}}}}

%%% Parametric extendible arrow %%%

% The following is commented out because of clash with mathtools package
%\newcommand{\xRightarrow}[2]{%
%  \ext@arrow3399{\longrightarrowtfill@}{#1}{#2}}
\newcommand{\longrightarrowtfill@}{%
  \arrowfill@\Relbar\Relbar\Rightarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\larg}[2]{#1.\text{arg}_{#2}}
\newcommand{\largn}[1]{\operatorname{arity}(#1)}


\newcommand{\Data}{\dom{Data}}
% \newcommand{\Terms}{\mathcal{T}_\Constr}

\newcommand{\Vars}{\mathcal{V}}
\newcommand\order{\operatorname{ord}}
\newcommand\FV{\mathit{FV}}

\newcommand{\Prog}{\ensuremath{\mathcal{P}}}
\newcommand\var{\operatorname{var}}

\newcommand{\rulename}[1]{\textbf{\textit{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ACS abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Acs}{\ensuremath{\mathcal{A}}}
\newcommand{\VAS}{\ensuremath{\mathcal{V}}}
\newcommand{\transto}{\mathrel{\rightarrowtail}}

%\newcommand{\ecsrule}[4][\pid]{(#1,\ #2,\ #3,\ #4)}
\newcommand{\ecsrule}[4][\pid]{#1\colon #2\xrightarrow{#3}#4}

\def\eTau#1[#2-->#3]{\ecsrule[\ifx!#1!\pid\else #1\fi]{#2}{\tau}{#3}}
\def\eSend#1[#2--#3!#4-->#5]{\ecsrule[\ifx!#1!\pid\else #1\fi]{#2}{#3\mathbin{!}#4}{#5}}
\def\eRec#1[#2--?#3-->#4]{\ecsrule[\ifx!#1!\pid\else #1\fi]{#2}{?#3}{#4}}
\def\eSpawn#1[#2--v#3.#4-->#5]{\ecsrule[\ifx!#1!\pid\else #1\fi]{#2}{\nu#3.#4}{#5}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Erlang semantics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\fun}{\mathit{fun}}
\newcommand{\pat}{\mathit{pat}}

% Constructs (for out of listing env use)
\newcommand{\Rec}{\erl[columns=fullflexible]{receive}}
\newcommand{\Send}[2]{\erl[columns=fullflexible]{send}(#1, #2)}
\newcommand{\Spawn}[3][]{\erl[columns=fullflexible]{spawn}\ensuremath{_{#1}}\ #2\ #3}
\newcommand{\Self}{\erl[columns=fullflexible]{self}}

% Processes

%% \proc to be used only in informal semantics
\newcommand{\proc}[3]{\tuple{#1}^{#2}_{#3}} % exp pid queue

\newcommand{\pid}{\iota}
\newcommand{\timest}{\vartheta}
\newcommand{\cntr}{t} % contour!

% Generic operations
\newcommand{\cons}{\mathbin{\cdot}}
\newcommand{\eseq}{\ensuremath{\epsilon}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract Machine
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dom}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\ProgLoc}{\dom{ProgLoc}}
\newcommand{\Exp}{\dom{Exp}}
\newcommand{\Constr}{\Sigma}
\newcommand{\Val}{\dom{Value}}
\let\Value\Val
\newcommand{\State}{\dom{State}}
\newcommand{\Store}{\dom{Store}}
\newcommand{\ProcState}{\dom{ProcState}}
\newcommand{\Procs}{\dom{Procs}}
\newcommand{\Mailbox}{\dom{Mailbox}}
\newcommand{\Mailboxes}{\dom{Mailboxes}}
\newcommand{\Closure}{\dom{Closure}}
\newcommand{\Env}{\dom{Env}}
\newcommand{\Var}{\dom{Var}}

\newcommand{\TimeStamp}{\dom{TimeSt}}
\newcommand{\Time}{\dom{Time}}
\newcommand{\Contour}{\dom{Time}}
\newcommand{\Pid}{\dom{Pid}}

\newcommand{\Addr}{\dom{Addr}}
\newcommand{\AddrKont}{\dom{KAddr}}
\newcommand{\AddrVar}{\dom{VAddr}}
\let\AddrVal\AddrVar % alias in case of confusion
\newcommand{\Msg}{\ensuremath{\widehat{\dom{Msg}}}}

\newcommand{\Kont}{\dom{Kont}}

%\newcommand{\Pat}{\dom{Pat}}

\newcommand{\finmap}{\rightharpoonup}
\newcommand{\fundom}{\operatorname{dom}}
\newcommand{\undef}[2]{#1(#2) = \bot}

\newcommand{\match}{\operatorname{match}}

\newcommand{\msg}{\ensuremath{m}}
\newcommand{\mailbox}{\ensuremath{\mathfrak{m}}}
\newcommand{\emptymb}{\ensuremath{\epsilon}}
\newcommand{\emptycntr}{\ensuremath{\epsilon}}

\newcommand{\data}{\delta}
\newcommand{\databot}{\_}

\newcommand{\mailmatch}{\operatorname{mmatch}}
%\newcommand{\enqueue}{\operatorname{enqueue}}
\newcommand{\enqueue}{\operatorname{enq}}
% \newcommand{\newKaddr}{\operatorname{new}_{ka}}
\newcommand{\newKPush}{\operatorname{new}_{\text{kpush}}}
\newcommand{\newKPop}{\operatorname{new}_{\text{kpop}}}
\newcommand{\newVaddr}{\operatorname{new}_{\text{va}}}
\newcommand{\newpid}{\operatorname{new}_{\text{pid}}}
\let\newPid\newpid
\newcommand{\tick}{\operatorname{tick}}

\newcommand{\kont}{\ensuremath{\kappa}}
\newcommand{\kontTag}[1]{\text{\sffamily #1}}
\newcommand{\kontData}[2]{\kontTag{#1}\tuple{#2}}
\newcommand{\kTop}{\text{\sffamily Stop}}
\let\kStop\kTop % unfortunate choice of macro name
\newcommand{\kArg}[1]{\kontData{Arg$_{#1}$}}
% \newcommand{\kMsg}{\kontData{Msg}}
% \newcommand{\kDispatch}{\kontData{Dispatch}}
% \newcommand{\kNewProc}{\kontData{NewPr}}
\newcommand{\kCase}{\kontData{Case}}

\newcommand{\resolve}[1][]{\operatorname{res}_{#1}}
\newcommand{\absresolve}[1][]{\widehat{\operatorname{res}}_{#1}}

\newcommand{\CFA}[1]{\mbox{#1-CFA}}
\newcommand{\zCFA}{\CFA{0}}
\newcommand{\kCFA}{\CFA{$k$}}
\newcommand{\kwCFA}{\textup{CFA($k$,$w$)}}

\newcommand{\semTo}{\to}
\newcommand{\cfaTo}{\leadsto}
\newcommand{\acsTo}{\to_{{\textup{acs}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract Interpretation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\AbsInt}{\mathcal{I}}
\newcommand{\DataAbs}{\mathcal{D}}
\newcommand{\TimeAbs}{\mathcal{T}}
\newcommand{\MailboxAbs}{\mathcal{M}}
\newcommand{\MsgAbs}{\mathcal{D}_{\text{msg}}}

\newcommand{\leqmb}[1][m]{\leq_{\text{#1}}}
\newcommand{\leqx}[1][]{\leq_{\text{#1}}}
\newcommand{\id}{\text{id}}
% ABS
%% Might style notation
\gdef\abs#1{\ifx\to#1\cfaTo\else\widehat#1\fi}
%% Cousot style notation
% \gdef\abs#1{\ifx\to#1\cfaTo\else{{#1}^{\sharp}}\fi}
%% Tilde notation
% \gdef\abs#1{\ifx\to#1\cfaTo\else\widetilde#1\fi}


\newcommand{\join}{\sqcup}
\newcommand{\bigjoin}{\bigsqcup}

\newcommand{\absf}[1][]{\alpha_{\text{#1}}}
\newcommand{\concf}[1][]{\gamma_{\text{#1}}}
\newcommand{\absfp}[1][ACS]{\alpha^{\text{pat}}_{\text{#1}}}
% \newcommand{\absfD}[1][ACS]{\alpha^{\text{D}}_{\text{#1}}}
\newcommand{\absfK}[1][ACS]{\alpha^{k}_{\text{#1}}}
% \newcommand{\absfM}[1][ACS]{\alpha^{\text{M}}_{\text{#1}}}

\newcommand{\hole}{\_}
% \newcommand{\hole}{\bullet}
\newcommand{\depthD}[2][D]{{\lfloor{#2}\rfloor}_{#1}}
% \newcommand{\depthD}[2][D]{{#2}|_{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Complexity classes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\complclass}{\textsc}
\newcommand{\expspace}{\complclass{Expspace}}
\newcommand{\exptime}{\complclass{Exptime}}
\newcommand{\ptime}{\complclass{P}}
\newcommand{\pspace}{\complclass{Pspace}}
\newcommand{\np}{\complclass{NP}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typesetting of operational semantic tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\colwd}

%
% Luke: I have changed ''when'' to ''if''
%
\newcommand{\CondCell}[2][if]{%
	\parbox[t]{\colwd}{#1\space$\begin{array}[t]{@{}r@{\;}l@{}}#2\end{array}$}}

\newcommand{\ResCell}[2][then]{%
	\parbox[t]{\colwd}{#1\space$\begin{array}[t]{@{}r@{\;}l@{}}#2\end{array}$}}

\newcounter{RULE}
\newcommand{\formatRuleName}[1]{\textbf{\small #1}}
\newcommand{\RuleName}[1]{%
	%\smallskip%
	\formatRuleName{#1}%
	\renewcommand{\theRULE}{\formatRuleName{#1}}%
	\refstepcounter{RULE}%
}

\newcommand{\ARN}[1]{Abs#1}
\newcommand{\AbsRuleName}[1]{%
	\smallskip%
	\formatRuleName{\ARN{#1}}%
	\renewcommand{\theRULE}{\formatRuleName{\ARN{#1}}}%
	\refstepcounter{RULE}%
}

\newcommand{\RulesSection}[1]{\textbf{\color{red!40!black}#1}}

\newcommand{\atom}[1]{\text{\texttt{\color{atom}#1}}}

\newcommand{\StopAddr}{\boldsymbol{\ast}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Syntax environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begingroup
\catcode`\|=\active%
\gdef\@redefbar{%
    \catcode`\|=\active%
    \def|{\hspace{3pt}\mid\hspace{3pt}}
}
\endgroup

\newenvironment{syntax}{%
    \begin{equation*}
    \def\prod{\mathrel{::=}}
    \renewcommand{\arraystretch}{1.2}
    \@redefbar
    \begin{array}{rl}%
}
{%
    \end{array}
    \end{equation*}
}
\let\grammar\syntax
\let\endgrammar\endsyntax

\makeatother

